Controlling Repetition in Protein Language Models

Protein language models (PLMs) have enabled advances in structure prediction and de novo protein design, yet they frequently collapse into pathological repetition during generation. Unlike in text, where repetition merely reduces readability, in proteins it undermines structural confidence and functional viability. To unify this problem, we present the first systematic study of repetition in PLMs. We first propose quantitative metrics to characterize motif-level and homopolymer repetition and then demonstrate their negative impact on folding reliability. To address this challenge, we propose UCCS (Utility-Controlled Contrastive Steering), which steers protein generation with a constrained dataset. Instead of naively contrasting high- vs. low-repetition sequences, we construct contrastive sets that maximize differences in repetition while tightly controlling for structural utility. This disentanglement yields steering vectors that specifically target repetition without degrading foldability. Injected at inference, these vectors consistently reduce repetition without retraining or heuristic decoding. Experiments with ESM-3 and ProtGPT2 in CATH, UniRef50, and SCOP show that our method outperforms decoding penalties and other baselines, substantially lowering repetition while preserving AlphaFold confidence scores. Our results establish repetition control as a central challenge for PLMs and highlight dataset-guided steering as a principled approach for reliable protein generation.

==> tables/experiment/main.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.15}
\caption{ESM3 results for two tasks with utility constraint: (a) unconditional generation, (b) conditional generation.\protect\footnotemark}
\label{tab:main-esm3}\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l *{3}{r r}}
\toprule
\multirow{2}{*}{\textbf{Method}}  & \multicolumn{2}{c}{\textbf{CATH}}  & \multicolumn{2}{c}{\textbf{UniRef50}}  & \multicolumn{2}{c}{\textbf{SCOP}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & {$R \uparrow$} & {$U \uparrow$} & {$R \uparrow$} & {$U \uparrow$} & {$R \uparrow$} & {$U \uparrow$} \\
\midrule
\textbf{(a) Unconditional generation}\\
Original Model & 
\label{tab:main-esm3-uncond}
$0.423\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.024}}$ & $0.576\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.027}}$ \good{} & $0.423\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.024}}$ & $0.576\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.027}}$ \good{} & $0.423\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.024}}$ & $0.576\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.027}}$ \good{} \\
Temperature Sampling & $0.751\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ & $0.566\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ & $0.751\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ & $0.566\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ & $0.751\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ & $0.566\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ \\
Top-p Sampling & $0.419\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.030}}$ & $0.590\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.037}}$ \good{} & $0.419\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.030}}$ & $0.590\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.037}}$ \good{} & $0.419\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.030}}$ & $0.590\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.037}}$ \good{} \\
Entropy Based Sampling & $\mathbf{0.904}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.002}}$ & $0.477\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $\mathbf{0.904}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.002}}$ & $0.477\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $\mathbf{0.904}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.002}}$ & $0.477\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ \\
Neuron Deactivation & $0.551\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.071}}$ & $0.507\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.048}}$ & $0.448\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.040}}$ & $0.594\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ \good{} & $0.452\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.020}}$ & $0.597\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.035}}$ \good{} \\
Probe Steering & $0.415\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.587\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ \good{} & $0.416\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.586\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ \good{} & $0.415\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.585\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ \good{} \\
UUCS(ours) & $0.645\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $\mathbf{0.652}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.020}}$ \good{} & $0.631\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.016}}$ & $\mathbf{0.646}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ \good{} & $0.641\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $\mathbf{0.646}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ \good{} \\
\addlinespace[3pt]
\midrule
\textbf{(b) Conditional generation}\\
Original Model & 
\label{tab:main-esm3-cond}
$0.542\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $0.686\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} & $0.542\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $0.686\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} & $0.542\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $0.686\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} \\
Temperature Sampling & $0.792\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ & $0.652\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ & $0.792\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ & $0.652\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ & $0.792\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ & $0.652\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ \\
Top-p Sampling & $0.539\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.016}}$ & $0.681\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $0.539\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.016}}$ & $0.681\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $0.539\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.016}}$ & $0.681\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ \\
Entropy Based Sampling & $\mathbf{0.923}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.003}}$ & $0.578\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ & $\mathbf{0.923}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.003}}$ & $0.578\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ & $\mathbf{0.923}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.003}}$ & $0.578\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ \\
Neuron Deactivation & $0.637\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.024}}$ & $0.636\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.031}}$ & $0.590\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.100}}$ & $0.638\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $0.557\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.673\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.030}}$ \\
Probe Steering & $0.546\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.005}}$ & $0.685\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.024}}$ & $0.546\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.005}}$ & $0.685\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ & $0.546\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.005}}$ & $0.686\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.023}}$ \\
UUCS(ours) & $0.707\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.019}}$ & $\mathbf{0.720}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ \good{} & $0.707\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ & $\mathbf{0.726}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ \good{} & $0.707\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ & $\mathbf{0.717}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} \\
\addlinespace[3pt]
\bottomrule
\end{tabular}
}
\vspace{-12pt}
\end{table}

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.15}
\caption{ProtGPT2 results for two tasks with utility constraint: (a) unconditional generation, (b) conditional generation. \protect\footnotemark[\value{footnote}]}
\label{tab:main-protgpt2}\vspace{-5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l *{3}{r r}}
\toprule
\multirow{2}{*}{\textbf{Method}}  & \multicolumn{2}{c}{\textbf{CATH}}  & \multicolumn{2}{c}{\textbf{UniRef50}}  & \multicolumn{2}{c}{\textbf{SCOP}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & {$R \uparrow$} & {$U \uparrow$} & {$R \uparrow$} & {$U \uparrow$} & {$R \uparrow$} & {$U \uparrow$} \\
\midrule
\textbf{(a) Unconditional generation}\\
Original Model & 
\label{tab:main-protgpt2-uncond}
$0.728\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.621\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ \good{} & $0.728\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.621\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ \good{} & $0.728\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.621\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ \good{} \\
Temperature Sampling & $0.756\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $0.612\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.019}}$ & $0.756\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $0.612\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.019}}$ & $0.756\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $0.612\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.019}}$ \\
Top-p Sampling & $0.714\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.608\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ & $0.714\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.608\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ & $0.714\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.608\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ \\
No Repeat N-gram & $0.736\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.613\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ & $0.736\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.613\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ & $0.736\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.613\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \\
Repetition Penalty & $0.780\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.003}}$ & $0.622\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} & $0.780\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.003}}$ & $0.622\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} & $0.780\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.003}}$ & $0.622\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} \\
Neuron Deactivation & $0.719\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.017}}$ & $0.610\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.718\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.019}}$ & $0.614\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.029}}$ & $0.734\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.009}}$ & $0.615\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.015}}$ \\
Probe Steering & $0.722\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.017}}$ & $0.607\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.017}}$ & $0.732\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.015}}$ & $0.624\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.029}}$ \good{} & $0.735\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.017}}$ & $0.619\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.016}}$ \\
UUCS(ours) & $\mathbf{0.845}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $\mathbf{0.711}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.004}}$ \good{} & $\mathbf{0.824}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ & $\mathbf{0.703}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ \good{} & $\mathbf{0.835}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ & $\mathbf{0.722}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ \good{} \\
\addlinespace[3pt]
\midrule
\textbf{(b) Conditional generation}\\
Original Model & 
\label{tab:main-protgpt2-cond}
$0.836\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ & $0.704\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.023}}$ \good{} & $0.836\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ & $0.704\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.023}}$ \good{} & $0.836\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.018}}$ & $0.704\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.023}}$ \good{} \\
Temperature Sampling & $0.847\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.700\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ & $0.847\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.700\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ & $0.847\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.700\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ \\
Top-p Sampling & $0.827\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $0.710\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ \good{} & $0.827\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $0.710\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ \good{} & $0.827\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ & $0.710\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ \good{} \\
No Repeat N-gram & $0.828\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.708\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.025}}$ \good{} & $0.828\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.708\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.025}}$ \good{} & $0.828\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.708\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.025}}$ \good{} \\
Repetition Penalty & $0.843\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.716\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ \good{} & $0.843\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.716\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ \good{} & $0.843\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ & $0.716\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.021}}$ \good{} \\
Neuron Deactivation & $0.836\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ & $0.709\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.012}}$ \good{} & $0.828\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.009}}$ & $0.706\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.015}}$ \good{} & $0.827\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.004}}$ & $0.701\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ \\
Probe Steering & $0.829\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.019}}$ & $0.702\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.020}}$ & $0.829\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.009}}$ & $0.690\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.010}}$ & $0.824\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ & $0.686\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.006}}$ \\
UUCS(ours) & $\mathbf{0.877}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.009}}$ & $\mathbf{0.743}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.013}}$ \good{} & $\mathbf{0.880}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.011}}$ & $\mathbf{0.725}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.022}}$ \good{} & $\mathbf{0.890}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.008}}$ & $\mathbf{0.737}\smash{\raisebox{-0.6ex}{\scriptsize$\pm$0.014}}$ \good{} \\
\addlinespace[3pt]
\bottomrule
\end{tabular}
}
\vspace{-12pt}
\end{table}


==> tables/main_table.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{Main results across tasks and scenarios.}
\label{tab:main}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.05}
\begin{threeparttable}
\begin{tabular}{l l l ccc cc ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Task} & \multirow{2}{*}{Scenario} &
\multicolumn{3}{c}{Repetition} &
\multicolumn{2}{c}{Bio Util.} &
\multicolumn{3}{c}{Method-level Macro} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-11}
& & &
rep. $\downarrow$ & hpoly. $\downarrow$ & $entropy \uparrow$ &
pLDDT $\uparrow$ & pTM $\uparrow$ &
$GM_{\text{rep}}\uparrow$ & $GM_{\text{bio}}\uparrow$ & Overall \\
\midrule
\multirow{5}{*}{contrastive\_layer} & \multirow{2}{*}{Uncond} & Fixed length   & \textbf{0.26 $\pm$ 0.0052} & \textbf{6.92 $\pm$ 0.16} & \textbf{0.678 $\pm$ 0.0056} & \textbf{82.2 $\pm$ 0.27} & \textbf{0.571 $\pm$ 0.009} & \multirow{5}{*}{\textbf{70.11\%}} & \multirow{5}{*}{\textbf{8.29\%}} & \multirow{5}{*}{\textbf{1.297}} \\
&  & Uniform        & \textbf{0.313 $\pm$ 0.0025} & \textbf{8.36 $\pm$ 0.19} & \textbf{0.647 $\pm$ 0.0031} & \textbf{68.8 $\pm$ 0.73} & \textbf{0.424 $\pm$ 0.0077} &  &  &  \\
& \multirow{3}{*}{Cond} & \hspace{1em}5\%   & \textbf{0.24 $\pm$ 0.0043} & \textbf{5.96 $\pm$ 0.19} & \textbf{0.709 $\pm$ 0.0029} & \textbf{80.4 $\pm$ 0.96} & \textbf{0.543 $\pm$ 0.012} &  &  &  \\
&  & \hspace{1em}10\%        & \textbf{0.216 $\pm$ 0.0017} & \textbf{5.93 $\pm$ 0.18} & \textbf{0.732 $\pm$ 0.0045} & \textbf{81.3 $\pm$ 0.53} & \textbf{0.554 $\pm$ 0.0081} &  &  &  \\
&  & \hspace{1em}15\%        & \textbf{0.193 $\pm$ 0.0035} & \textbf{5.6 $\pm$ 0.13} & \textbf{0.761 $\pm$ 0.003} & \textbf{83 $\pm$ 0.51} & \textbf{0.583 $\pm$ 0.0065} &  &  &  \\
\midrule
\multirow{5}{*}{baseline(no steer)} & \multirow{2}{*}{Uncond} & Fixed length   & 0.462 $\pm$ 0.0065 & 15.3 $\pm$ 0.39 & 0.517 $\pm$ 0.0086 & 73.9 $\pm$ 0.44 & 0.521 $\pm$ 0.0089 & \multirow{5}{*}{0.00\%} & \multirow{5}{*}{0.00\%} & \multirow{5}{*}{1.0} \\
&  & Uniform        & 0.547 $\pm$ 0.012 & 22 $\pm$ 0.66 & 0.466 $\pm$ 0.01 & 58.4 $\pm$ 2.1 & 0.393 $\pm$ 0.015 &  &  &  \\
& \multirow{3}{*}{Cond} & \hspace{1em}5\%   & 0.422 $\pm$ 0.0092 & 14.3 $\pm$ 0.31 & 0.567 $\pm$ 0.0052 & 75.3 $\pm$ 0.95 & 0.521 $\pm$ 0.0062 &  &  &  \\
&  & \hspace{1em}10\%        & 0.364 $\pm$ 0.0025 & 12.8 $\pm$ 0.27 & 0.623 $\pm$ 0.0011 & 75.6 $\pm$ 0.69 & 0.524 $\pm$ 0.0085 &  &  &  \\
&  & \hspace{1em}15\%        & 0.316 $\pm$ 0.0088 & 11.7 $\pm$ 0.35 & 0.667 $\pm$ 0.0093 & 78.5 $\pm$ 0.46 & 0.549 $\pm$ 0.011 &  &  &  \\
\midrule
\multirow{5}{*}{neuron\_topk} & \multirow{2}{*}{Uncond} & Fixed length   & 0.458 $\pm$ 0.0093 & 15.1 $\pm$ 0.41 & 0.519 $\pm$ 0.0085 & 74 $\pm$ 0.42 & 0.515 $\pm$ 0.0057 & \multirow{5}{*}{-0.07\%} & \multirow{5}{*}{-1.10\%} & \multirow{5}{*}{0.993} \\
&  & Uniform        & 0.547 $\pm$ 0.012 & 21.8 $\pm$ 0.63 & 0.466 $\pm$ 0.011 & 57.7 $\pm$ 1.8 & 0.386 $\pm$ 0.012 &  &  &  \\
& \multirow{3}{*}{Cond} & \hspace{1em}5\%   & 0.423 $\pm$ 0.0091 & 14.1 $\pm$ 0.34 & 0.566 $\pm$ 0.0065 & 74.8 $\pm$ 0.67 & 0.512 $\pm$ 0.0037 &  &  &  \\
&  & \hspace{1em}10\%        & 0.366 $\pm$ 0.0044 & 12.8 $\pm$ 0.23 & 0.62 $\pm$ 0.0017 & 75.2 $\pm$ 0.5 & 0.525 $\pm$ 0.0071 &  &  &  \\
&  & \hspace{1em}15\%        & 0.322 $\pm$ 0.0074 & 11.8 $\pm$ 0.43 & 0.661 $\pm$ 0.0092 & 77.1 $\pm$ 0.39 & 0.535 $\pm$ 0.0078 &  &  &  \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}






% \begin{table*}[t]
% \centering
% \scriptsize
% \caption{Main results across tasks and scenarios.}
% \label{tab:main}
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{threeparttable}
% \begin{tabular}{l l l ccc cc ccc}
% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Task} & \multirow{2}{*}{Scenario} &
% \multicolumn{3}{c}{Repetition} &
% \multicolumn{2}{c}{Bio Util.} &
% \multicolumn{3}{c}{Method-level} \\
% \cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-11}
% & & &
% rep. $\downarrow$ & hpoly. $\downarrow$ & $H \uparrow$ &
% pLDDT $\uparrow$ & pTM $\uparrow$ &
% $GM_{\text{rep}}\uparrow$ & $GM_{\text{bio}}\uparrow$ & Overall \\
% \midrule
% \multirow{5}{*}{Control}
% & \multirow{2}{*}{Uncond} & Fixed length   &  &  &  &  &  & \multirow{5}{*}{} & \multirow{5}{*}{} & \multirow{5}{*}{} \\
% &                          & Uniform        &  &  &  &  &  &                     &                     &                     \\
% & \multirow{3}{*}{Cond} 
% & \hspace{1em}5\%   &  &  &  &  &  &                     &                     &                     \\
% & & \hspace{1em}10\% &  &  &  &  &  &                     &                     &                     \\
% & & \hspace{1em}15\% &  &  &  &  &  &                     &                     &                     \\
% \midrule
% \multirow{5}{*}{\textit{YourMethod}}
% & \multirow{2}{*}{Uncond} & Fixed length   &  &  &  &  &  & \multirow{5}{*}{} & \multirow{5}{*}{} & \multirow{5}{*}{} \\
% &                          & Uniform        &  &  &  &  &  &                     &                     &                     \\
% & \multirow{3}{*}{Cond} 
% & \hspace{1em}5\%   &  &  &  &  &  &                     &                     &                     \\
% & & \hspace{1em}10\% &  &  &  &  &  &                     &                     &                     \\
% & & \hspace{1em}15\% &  &  &  &  &  &                     &                     &                     \\
% \bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

==> tables/statics_raw_data.tex <==
\begin{table}[t]
\centering
\caption{Dataset-level statistics (means across sequences). Lower values indicate worse performance for all reported metrics.}
\label{tab:dataset-metrics}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
Dataset & N & Avg Len & $H_{\mathrm{norm}}(x)$ & $\mathrm{Distinct}\!-\!n(x)$ & $R_{\mathrm{hpoly}}(x)$ & $\mathrm{pLDDT}(x)$ & $\mathrm{pTM}(x)$ \\
\midrule
ESM-raw-neg & 10000 & 541.8 & \textbf{0.436} & \textbf{0.208} & \textbf{0.516} & \textbf{0.634} & \textbf{0.427} \\
CATH & 9998 & 157.5 & 0.917 & 0.867 & 0.994 & 0.899 & 0.763 \\
UniProt & 9895 & 324.9 & 0.926 & 0.781 & 0.996 & 0.901 & 0.767 \\
SCOP & 9868 & 195.4 & 0.924 & 0.850 & 0.999 & 0.916 & 0.811 \\
\bottomrule
\end{tabular}
}
\vspace{-7pt}
\end{table}

